Dynamic Transition From Mach to Regular Reflection Over a Moving Wedge

The design of supersonic and hypersonic air-breathing vehicles is influenced by the transition between the Mach Reflection (MR) and Regular Reflection (RR) phenomena. The purpose of this study is to investigate the dynamic transition of unsteady supersonic flow from MR to RR over a two-dimensional wedge numerically. The trailing edge of the wedge moves downstream along the $x$-direction with a velocity, $V(t)$ at a free-stream Mach number of $3$. An unsteady compressible inviscid flow solver is used to simulate the phenomenon. Further, the Arbitrary Lagrangian-Eulerian (ALE) technique is applied to deform the mesh during the wedge motion. The dynamic transition from MR to RR is defined by two criteria, the sonic and the Von-Neumann. Moreover, the lag in the dynamic transition from the steady-state condition is studied using various reduced frequencies, $\kappa$, in the range of [0.1-2]. The lag effect in the shock system is remarkable at the high values of the reduced frequency, $\kappa=1.5$ and $2.0$. Furthermore, because the shock is bent upstream during the fast motion of the wedge, the transition from MR to RR happens below the Dual Solution Domain (DSD).

==> 00_Abstract_Extended.tex <==
\textit{Moving wedge in a high-speed flow represents one of the aerodynamic flow controls for the supersonic and hypersonic air-breathing vehicles. The transition between the regular reflection and Mach reflection phenomenon, which impacts the design of these vehicles, would be affected by the wedge's motion. The aim of this paper is to numerically investigate the dynamic transition from regular reflection to Mach reflection of unsteady supersonic flow. The phenomenon is studied over a two-dimensional wedge whose trailing edge moves along the $x$-direction upstream with a velocity, $V(t)$ at a free-stream Mach number of $M_{\infty}=3$. Thus, the wedge's height, $H$, is kept fixed, but its length, $L(t)$, decreases during the movement of the wedge from its initial location. The simulation is conducted using the unsteady compressible inviscid flow solver, which is implemented in OpenFOAM\textsuperscript{\textregistered}, the open-source CFD tool. Further, the wedge motion is applied by moving the mesh boundary, performing the Arbitrary Lagrangian-Eulerian (ALE) technique. This was achieved by integrating a written $C$++ code of the wedge's motion with the flow solver, (rhoCentralDyMFoam). Then, the precision of the computational simulations was determined using a mesh-independent study. In addition, the sonic and the detachment criteria are used to define the dynamic transition from regular reflection to Mach reflection during the increase of the wedge angle from $19^{\circ}$ to $27^{\circ}$. Different non-dimensional angular velocities, $\kappa$, in the range of $[0.1-1]$ for the moving wedge are applied to study the lag in the dynamic transition from the steady-state condition. The lag is analyzed by measuring the flow characteristic parameters, such as wedge angle, $\theta_w$, the tangent wave angle at the wedge's leading-edge, $\beta_t$, and the incident wave angle at the reflection point, $\beta$, at the selected transition criteria from regular reflection to Mach reflection for each non-dimensional angular velocity. Further, the variation of the Mach stem height is measured during increasing the wedge angle. The results show that the detachment criterion occurs within $1.5^{\circ}$ after the sonic criterion. At low-frequency rates of wedge motion, the transition occurs close to the theoretical limit. However, the lag in transition increases and the Mach stem height decreases as the wedge moves at higher frequency rates. In addition, the transition from regular reflection to Mach reflection occurs above the Dual Solution Domain (DSD), since the shock is curved downstream during the rapid motion of the wedge. }

==> 1_Nomenclature.tex <==
\mbox{}
\nomenclature[B]{$\kappa$}{Non-dimensional angular velocity}
\nomenclature[A]{$L(t)$}{Wedge stream-wise length}
%\nomenclature[A]{$L_{t}$}{the length of the wedge plus flat plate }
\nomenclature[A]{$w(t)$}{Wedge chord}
\nomenclature[A]{$\tau$}{Non-dimensional time}
\nomenclature[A]{$\theta(t)$}{Wedge angle}
\nomenclature[A]{$h$}{Wedge height}
%\nomenclature[A]{$M_{\infty}$}{Free-stream Mach number}
%\nomenclature[A]{$M_t(t)$}{Trailing-edge Mach number}
\nomenclature[A]{$V_t(t)$}{Trailing-edge velocity}
\nomenclature[A]{$\mathrm{MS}$}{Mach stem height}
\nomenclature[A]{$H$}{Half height of computational inflow boundary}
%\nomenclature[A]{$v$}{Velocity component in $y$-direction}
%\nomenclature[A]{$\rho$}{Flow field density}
%\nomenclature[A]{$p$}{Flow field pressure}
\nomenclature[B]{$\beta_{p}$}{Incident wave angle at reflection$/$triple point}
\nomenclature[B]{$\beta_{tang}$}{Tangent wave angle at wedge's apex}
\nomenclature[B]{$\beta_{t}$}{Transition wave angle}
\printnomenclature[0.68in]




